Real-Time Simulation of Open Quantum Spin Chains with Inchworm Method

We study the real-time simulation of open quantum systems, where the system is modeled by a spin chain, with each spin associated with its own harmonic bath. Our method couples the inchworm method for the spin-boson model and the modular path integral methodology for spin systems. In particular, the introduction of the inchworm method can significantly suppress the numerical sign problem. Both methods are tweaked to make them work seamlessly with each other. We represent our approach in the language of diagrammatic methods, and analyze the asymptotic behavior of the computational cost. Extensive numerical experiments are done to validate our method.

==> diagram_single_spin_boson.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=0.9]
\filldraw[fill=yellow] (0,0) circle (1cm);
\node[text=black] at (0,0) {$H_s$};
\filldraw[fill=green] (0,-4) circle (1cm);
\node[text=black] at (0,-4) {$H_b$};
\draw[dashed] (0,-1) -- (0,-3);
\node[text=black] at (0,-2) {$W_s\otimes W_b$};
\end{tikzpicture}
\caption{Illustration of a single spin coupled with a harmonic bath. The yellow circle stands for the spin and the green circle stands for its harmonic bath. The dashed line between a yellow circle and a green circle stands for the coupling relation between a spin and its bath.}
\label{diagram_spin_boson_model}
\end{figure}


==> dyson_series_inchworm_algorithm.tex <==
\label{sec_dyson_inchworm}
In this section, 
 we review the Dyson series and Inchworm algorithm for the spin-boson model.
It corresponds to the case when $n=1$ in \Cref{sec_model}.

We start from a toy ordinary differential equation model
\begin{equation}
    \dv{u(t)}{t} = (A+B) u(t)
\end{equation}
where $A, B$ are two constant operators.
The solution to this ODE can be given by
$u(t) = \e^{(A+B)t} u(0)$.
Multiplying both sides of the ODE and taking the integration over variable $t$ yields
\begin{equation}
    u(t) = \e^{At} u(0) + \int_{0}^t \e^{A(t-s_1)}Bu(s_1) \dd s_1.
\end{equation}
If we insert this equation to itself repeatly,
 under some certain convergence condition,
 we have
\begin{equation}
    u(t) = \e^{At} u(0)
    + \sum_{m=1}^{\infty}
    \int_{0\leqslant \boldsymbol{s} \leqslant t} \dd \boldsymbol{s} 
    \left[\e^{A(t-s_m)} B \e^{A(s_{m}-s_{m-1})} B \dots B \e^{A(s_2-s_1)} B \e^{As_1} u(0)\right],
\end{equation}
where 
\begin{equation}
    \int_{0\leqslant \boldsymbol{s} \leqslant t} \dd \boldsymbol{s} \text{(integrand)} 
    = \int_0^{t}\dd s_{m} \int_0^{s_{m-1}} \dd s_{m-1} \dots \int_0^{s_2} \dd s_1 \text{(integrand)}
\end{equation}
is the integral over an $m$-dimensional simplex.
Therefore, an expansion for the exponential operator $\e^{(A+B)t}$ is given by
\begin{equation}
\label{General_Dyson_Series}
    \e^{(A+B)t}
    = \e^{At} + \sum_{m=1}^{\infty}
    \int_{0\leqslant{s}\leqslant t}
    \dd \boldsymbol{s}
    \left[
    \e^{A(t-s_m)} B \e^{A(s_m-s_{m-1})} B \dots
    B \e^{A(s_2-s_1)} B \e^{As_1}
    \right].
\end{equation}
This expansion is called Dyson series 
 and it is originally developed and commonly used in quantum mechanics \cite{dyson1949radiation}.
This expression is a perturbative expansion to investigate the difference between $\e^{(A+B)t}$ and $\e^{At}$.

For the model discussed in \cref{sec_model}, 
 if the number of spins is $n=1$,
the system becomes one single spin coupled with a harmonic bath.
In this case, the total Hamiltonian becomes
\begin{equation}
    H = H_s + H_b + W_s \otimes W_b
\end{equation}
where
\begin{equation}
    H_s = \epsilon \sigma_z + \Delta \sigma_x, \quad
    H_b = \sum_{j} \frac{1}{2}\left(
    \hat{p}_j^2 
    + \omega_j^2 \hat{q}_j^2 \right), \quad
    W_s = \sigma_z,  \quad
    W_b = c_j  \hat{q}_j.
\end{equation}
The total Hamiltonian can then be represented by \Cref{diagram_spin_boson_model}.
\input{diagram_single_spin_boson.tex}
We may apply the Dyson series expansion to to the von Neumann equation
\begin{equation}
    \dv{\rho(t)}{t} = -\ii (H\rho(t) - \rho(t)H),
\end{equation}
because its solution can be
formatically expressed by $\rho(t) = \e^{-\ii H t}\rho(0) \e^{\ii H t}$
and $H$ is the sum of $H_s$ and $H_b + W_s\otimes W_b$.
Additionally, we only focus on some observable $O_s$ over the system of interest (the spin).
The expectation of the observable is given by
\begin{equation}
    \expval{O_s(t)} = \tr(O_s\rho(t))
    = \tr_s (\rho_s(0) G(-t,t))
\end{equation}
where the propagator $G(-t,t)$ is defined by
\begin{equation}
    G(-t,t)=\tr_b\left(\rho_b(0)\e^{\ii Ht O_s \e^{-\ii Ht}}\right).
\end{equation}
The application of Dyson expansion \cref{General_Dyson_Series} and the Wick's theorem \cite{wick1950evaluation,Negele1988} yields the following Dyson series expansion for the propagator $G(-t,t)$:
\begin{equation}
\label{fullPropagator}
    G(-t,t) = \e^{\ii t H_s} \hat{O}_s \e^{-\ii t H_s}
    + \sum_{m=1}^{\infty}
    \ii^m
    \int_{-t\leqslant \boldsymbol{s} \leqslant t}
    \dd \boldsymbol{s}
    \left[(-1)^{\#\{\boldsymbol{s}<0\}}
    \mathcal{U}^{(0)} (-t,\boldsymbol{s},t)
    \mathcal{L}_b(\boldsymbol{s})\right] \text{~for~} t \geqslant 0, 
\end{equation}
In the integrand, the notation $\#\{\boldsymbol{s}<0\}$ denotes the number of negative components 
in $\boldsymbol{s} = (s_1,\cdots,s_m)$, and
$\mathcal{U}^{(0)}(-t,\boldsymbol{s},t)$ describes the contribution of the system dynamics, which is defined by
\begin{equation}
    \label{U0}
    \mathcal{U}^{(0)} (-t,\boldsymbol{s},t)
    = G_s^{(0)}(s_m,t) W_s
    G_s^{(0)}(s_{m-1},s_m) W_s
    \cdots
    W_s G_s^{(0)}(s_1,s_2) 
    W_s G_s^{(0)}(-t,s_1)
\end{equation}
where
\begin{equation}
    G_s^{(0)} (s_\ii,s_\ff)
    = \begin{cases}
    \e^{-\ii (s_\ff-s_\ii)H_s}, 
    &\text{if }s_\ii \leqslant s_\ff < 0 \\
    \e^{-\ii (s_\ii-s_\ff)H_s},
    &\text{if }0 \leqslant s_\ii \leqslant s_\ff\\
    \e^{\ii s_\ff H_s}\hat{O}_s \e^{\ii s_\ii H_s},
    &\text{if } s_\ii < 0 \leqslant s_\ff
    \end{cases}.
    \label{Gs0_definition}
\end{equation}
The bath influence functional $\mathcal{L}_b$ satisfies the following Wick's theorem \cite{Negele1988}
\begin{equation}
\label{bath_influence_function_Lb}
    \mathcal{L}_b (s_1,\cdots,s_m) 
    = \begin{cases}
    0, & \quad\text{if $m$ is odd} \\
    \displaystyle\sum_{\mathfrak{q}\in\mathcal{Q}(\boldsymbol{s})}
    \prod_{(s_j,s_k)\in\mathfrak{q}}
    B(s_j,s_k), & \quad\text{if $m$ is even} 
    \end{cases}
\end{equation}
where $B(\tau_1,\tau_2)$ is a complex-valued functional
\begin{equation}
 \begin{split}
    B(\tau_1,\tau_2) =  B^*(\Delta \tau) = & \ \frac{1}{\pi}
    \int_0^{+\infty} J(\omega) \left[
    \coth\left(\frac{\beta\omega}{2}\right)
    \cos(\omega \Delta \tau) - \ii \sin(\omega \Delta \tau)
    \right]\dd \omega \\
    = & \   \frac{1}{2}\sum_j \frac{c_j^2}{\omega_j} 
    \left(
    \coth\left(\frac{\beta\omega_j}{2}\right)
    \cos(\omega_j \Delta \tau ) - \ii \sin(\omega_j \Delta \tau )
    \right)
     \end{split}
    \label{bath_function_B}
\end{equation}
with $\Delta \tau = \vert \tau_1 \vert - \vert \tau_2 \vert$.
The set $\mathcal{Q}(\boldsymbol{s})$ in \eqref{bath_influence_function_Lb} is given by
\begin{equation}
\label{Q}
\begin{split}
    \mathcal{Q}(s_1,\cdots,s_m)
    = \left.\Big\{
    \left\{
    (s_{j_1},s_{k_1}),\cdots,(s_{j_{m/2}},s_{k_{m/2}})   
    \right\}
    \right\vert&
    \{j_1,\cdots,j_{m/2},k_1,\cdots,k_{m/2}\} = \{1,\cdots,m\}, \\
    &j_l < k_l \text{ for any }l=1,\cdots,m/2
    \Big\}.
\end{split}
\end{equation}

The Dyson series \cref{fullPropagator}
 involves the integration over high dimensional simplices,
 which is computational expensive.
An effective method to reduce computational cost is to take the derivative with respect to time $t$,
 which yields
an integro-differential equation (see \cite{cai2022fast} for the derivation): 
\begin{equation}
    \frac{\dd }{\dd t}G(-t,t) = \ii [H_s,G(-t,t)] + W_s \mathcal{K}(-t,t) + \left(W_s \mathcal{K}(-t,t)\right)^\dagger, \qquad \forall t > 0,
  \label{integro_differential_eq}
\end{equation}
where $\mathcal{K}(-t,t)$ stands for the series:
\begin{equation}
\label{K_dyson}
\mathcal{K}(-t,t) \coloneqq \sum_{\substack{m=1 \\ m \text{~is odd}}}^{\infty}  \ii^{m+1} \int_{-t\leqslant \bs \leqslant t} \dd \bs  (-1)^{\#\{\bs < 0\}} \mathcal{U}^{(0)}(-t, \bs , t)  \mathcal{L}_s (\bs, t)
\end{equation}
and the initial condition is given by $G(0,0)=\hat{O}_s$ according to definition \eqref{fullPropagator}.

Another possible improvement is to replace bare propagator $G_s^{(0)}(s_\ii,s_\ff)$ 
by full propagator $G(s_\ii,s_\ff)$,
 which leads to the inchworm intego-differential equation \cite{cai2020inchworm,cai2022fast,cai2022bold} where $\mathcal{K}(-t,t)$ is rewritten as:
\begin{equation}
 \label{K inchworm}
 \mathcal{K}(-t,t) = \sum_{\substack{m=1 \\ m \text{~is odd}}}^{+\infty}  \ii^{m+1} \int_{-t\leqslant \bs \leqslant t} \dd \bs  (-1)^{\#\{\bs < 0\}} \mathcal{U}(-t, \bs , t)  \mathcal{L}_b^c(\bs,t)
\end{equation}
with
\begin{equation}
\begin{split}
   & \mathcal{U}(-t, s_1,\cdots,s_m , t) =   \ G(s_m,t) W_s
    G(s_{m-1},s_m) W_s
    \cdots
    W_s G(s_1,s_2) 
    W_s G(-t,s_1), \\
    & \mathcal{L}_b^c(s_1,\cdots,s_{m+1})  = \sum_{\mathfrak{q}\in\mathcal{Q}^c(s_1,\cdots,s_{m+1})}
    \prod_{(s_j,s_k)\in\mathfrak{q}}
    B(s_j,s_k)
\end{split}
\end{equation}
where $\mathcal{Q}^c \subset \mathcal{Q}$
represents all connected pairings.
For more details, please refer to \cite{cai2020inchworm}.

In conclusion,
 for a single spin-bath coupling,
 the bath influence functional $\mathcal{L}_b$ in Dyson series or $\mathcal{L}_b^c$ in Inchworm algorithm describe the influence of the bath to the system.
The system-associated part $\mathcal{U}^{(0)}(-t,\boldsymbol{s},t)$ or $\mathcal{U}(-t,\boldsymbol{s},t)$
 has similar form to the toy model of Dyson expansion in \cref{General_Dyson_Series}.



==> inchworm_each_spin_new.tex <==
In this section, we proposed a new algorithm for the computation of $\mathcal{G}^{(k)}(\boldsymbol{s})$ for given $\bs$ for a single spin.
The algorithm is inspired by the inchworm Monte Carlo Method for system-bath coupling \cite{chen2017inchworm1,chen2017inchworm2},
where a single heat bath interacts with entire system.

Since the baths are initially in the thermal equilibrium state, Wick's Theorem \cite{wick1950evaluation} can be applied to take the trace with respect to the bath part:
\begin{equation}
    \tr \left(
    \rho^{(k)}(t) \mathcal{G}^{(k)}(\bs)
    \right)
    = \tr_{s^{(k)}} \hspace{-4pt}
    \left[
        \rho_s^{(k)}(t)
        \left(\prod_{n=1}^N \sqrt{\ii \, \sgn(s_n)} \right)
        \sum_{M=0}^{\infty} \ii^M \hspace{-4pt}
        \int_{-t \leqslant \boldsymbol{\tau} \leqslant t}
        \left( \prod_{m=1}^M \ii \, \sgn(\tau_m) \right)
            \mathcal{U}_0^{(k)}(\boldsymbol{\tau},\boldsymbol{s})
            \mathcal{L}_b^{(k)}(\boldsymbol{\tau})
        \dd \boldsymbol{\tau}
    \right].
\end{equation}
Then we define
\begin{equation}
    \mathscr{G}^{(k)}(-t,\boldsymbol{s},t)
    = \left(\prod_{n=1}^N \sqrt{\ii \, \sgn(s_n)} \right)
    \sum_{M=0}^{\infty} \ii^M
    \int_{-t \leqslant \boldsymbol{\tau} \leqslant t}
    \left( \prod_{m=1}^M \ii \, \sgn(\tau_m) \right)
        \mathcal{U}_0^{(k)}(\boldsymbol{\tau},\boldsymbol{s})
        \mathcal{L}_b^{(k)}(\boldsymbol{\tau})
    \dd \boldsymbol{\tau},
\end{equation}
which yields $\tr\left(\rho(t) \mathcal{G}^{(k)}(\bs) \right) = \tr_{s^{(k)}}\left(\rho_s^{(k)}(t) \mathscr{G}^{(k)}(-t,\bs,t) \right)$.

